Functional Reactive Programming with Effects, A More Permissive Approach

We introduce a functional reactive programming language that extends WORMHOLES, an enhancement of YAMPA with support for effects. Our proposal relaxes the constraint in WORMHOLES that restricts all resources to single-use. Resources are categorized into two kinds: input/output resources and internal resources. Input/output resources model interactions with the environment and follow constraints similar to those in WORMHOLES. Internal resources, on the other hand, enable communication between program components and can be used multiple times. We demonstrate that programs written in our language can be translated into equivalent effect-free YAMPA programs, ensuring that our approach remains compatible with existing functional reactive paradigms.

==> figures/Language/example/reference_overview.tex <==
\begin{figure}[ht]
  \centering
      
  \begin{tikzpicture}[scale=0.7]

    \node (getIS) at (-4,0) {};
    \node[get] (get) at (-2,0) {r};
    \node (getOS) at (0.5,0) {};
    \node (getE) at (-2,2) {};
    \node (getLegend) at (-2,-1.1) {$\Get\,r$};

    \draw[dfarrow] (getIS) to[edge label={$e_1$}, pos=0.5] (get);
    \draw[dfarrow, dashed] (getE) to[edge label={$e_2$}, pos=0.5] (get);
    \draw[dfarrow] (get)   to[edge label={$(e_1,e_2)$}, pos=0.5] (getOS);

    \node (setIS) at (1.7,0) {};
    \node[set] (set) at (4.2,0) {r};
    \node (setOS) at (6.2,0) {};
    \node (setE) at (4.2,2) {};
    \node (setLegend) at (4.2,-1.1) {$\Set\,r$};

    \draw[dfarrow] (setIS) to[edge label={$(e_1,e_2)$}, pos=0.5] (set);
    \draw[dfarrow, dashed] (set) to[edge label={$e_2$}, pos=0.5] (setE);
    \draw[dfarrow] (set)   to[edge label={$e_1$}, pos=0.5] (setOS);

    % \node[first, dashed, minimum height = 70 pt] (rbinder) at (10,0.5) {};
    % \node (rbinderIS) at (7.5,0) {};
    % \node[draw=black,fill=white, minimum height = 12 pt, minimum width = 17 pt,dashed] (name) at (9.2,1.25) {\small $r$};
    % \node[draw=black,fill=white, minimum height = 12 pt, minimum width = 17 pt] (val) at (9.8,1.25) {\small $e$};
    % \node[arr] (rbinderArr) at (10,0) {$t$};
    % \node (rbinderOS) at (12.5,0) {};
    % \node (rbinderLegend) at (10,-1.1) {$\rbinder{r}{t}$};

    % \draw[dfarrow] (rbinderIS) to[edge label={$e_i$}, pos=0.4] (rbinderArr);
    % \draw[dfarrow] (rbinderArr)   to[edge label={$e'_i$}, pos=0.6] (rbinderOS);

  \end{tikzpicture}
  
  \caption{Graphical representation of resource accesses}
  \label{figure:reference:overview}
\end{figure}


==> figures/yampa/example/delay_wormholes.tex <==
\begin{figure}[ht]
  \vspace*{-3mm}

  \centering
      
  \begin{tikzpicture}[scale=0.7]

    \node[loopPre, minimum width = 300pt, minimum height = 150pt] (wormhole) at (1.5,0) {};


    \node (start) at (-5,0) {};
    \node (end) at (8,0) {};
    \node (c) at (-2,-2.1) {c$_{set}$};
    \node (c1) at (2,-2.1) {c$_{set}$};
    \node (c) at (1,2.1) {c$_{get}$};
    \node (c1) at (5,2.1) {c$_{get}$};
    \node[draw=black,fill=white,minimum width = 30pt,minimum height = 20pt,text=black!80] (cellset) at (-2.5,-1.5) {\texttt{unit}};
    \node[draw=black,fill=white,minimum width = 30pt,minimum height = 20pt,text=black!80] (cellset1) at (-1.5,-1.5) {\texttt{\_}};
    \node[draw=black,fill=white,minimum width = 30pt,minimum height = 20pt,text=black!80] (cellsetb) at (2.5,-1.5) {t};
    \node[draw=black,fill=white,minimum width = 30pt,minimum height = 20pt,text=black!80] (cellset1b) at (1.5,-1.5) {\texttt{\_}};


    \node[draw=black,fill=white,minimum width = 30pt,minimum height = 20pt,text=black!80] (cellget) at (0.5,1.5) {\texttt{v}};
    \node[draw=black,fill=white,minimum width = 30pt,minimum height = 20pt,text=black!80] (cellget1) at (1.5,1.5) {\texttt{\_}};
    \node[draw=black,fill=white,minimum width = 30pt,minimum height = 20pt,text=black!80] (cellgetb) at (5.5,1.5) {\texttt{unit}};
    \node[draw=black,fill=white,minimum width = 30pt,minimum height = 20pt,text=black!80] (cellget1b) at (4.5,1.5) {\texttt{\_}};

    \node[rsf] (rsfs) at (0,0) {$\rsf[r_{set}]$};
    \node[rsf] (rsfg) at (3,0) {$\rsf[r_{get}]$};


    \draw[dfarrow,dashed] (cellset1) to (-0.5,-0.55);
    \draw[dfarrow,dashed] (0.5,-0.55) to (cellset1b);
    \draw[-{Triangle[angle=45:4pt]},decorate,decoration={snake,amplitude=.4mm,segment length=2mm,post length=1mm}] (cellset1) to[edge label={\small update state}, pos=0.5] (cellset1b);

    \draw[dfarrow,dashed] (cellget1) to (2.5,0.55);
    \draw[dfarrow,dashed] (3.5,0.55) to (cellget1b);
    \draw[-{Triangle[angle=45:4pt]},decorate,decoration={snake,amplitude=.4mm,segment length=2mm,post length=1mm}] (cellget1) to[edge label={\small update state}, pos=0.5] (cellget1b);

    \draw[dfarrow] (rsfs) to[edge label={\small \void}, pos=0.5] (rsfg);
    \draw[dfarrow] (start) to[edge label={\small t}, pos=0.5] (rsfs);
    \draw[dfarrow] (rsfg) to[edge label={\small v}, pos=0.5] (end);

  \end{tikzpicture}
  
  \caption{Graphical representation the \texttt{delay} operation in \Wormholes.}
  \label{figure:example:wormholes:delay}
\end{figure}


==> figures/yampa/example/delay_yampa.tex <==
\begin{figure}[ht]

  \centering
      
  \begin{tikzpicture}[scale=0.7]

    \node (start) at (-3,0) {};
    \node (end) at (3,0) {};
    \node[loopPre, minimum width = 100pt] (loop) at (0,-0.2) {};
    \node[arr] (swap) at (0,0) {$\mathit{swap}$};
    \draw[dfarrow] (start) to[edge label={\small \texttt{t}}, pos=0.3] (swap);
    \draw[dfarrow] (swap) to[edge label={\small \texttt{v}}, pos=0.7] (end);
    \draw (swap) to[edge label={\small \texttt{(v,t)}}, pos=0.2] (end);
    \draw (start) to[edge label={\small \texttt{(t,v)}}, pos=0.8] (swap);
    \draw[rounded corners] (swap) -- (1.25,0) to[edge label={\small \texttt{t}}, pos=0.5] (1.25,-0.75) -- (-1.25,-0.75) to[edge label={\small \texttt{v}}, pos=0.5] (-1.25,0) -- (swap);

  \end{tikzpicture}
  
  \caption{Graphical representation the \texttt{delay v} operation in \Yampa.}
  \label{figure:example:yampa:delay}
\end{figure}
